Self-Contrastive Learning: Single-viewed Supervised Contrastive Framework using Sub-network

Contrastive loss has significantly improved performance in supervised classification tasks by using a multi-viewed framework that leverages augmentation and label information. The augmentation enables contrast with another view of a single image but enlarges training time and memory usage. To exploit the strength of multi-views while avoiding the high computation cost, we introduce a multi-exit architecture that outputs multiple features of a single image in a single-viewed framework. To this end, we propose Self-Contrastive (SelfCon) learning, which self-contrasts within multiple outputs from the different levels of a single network. The multi-exit architecture efficiently replaces multi-augmented images and leverages various information from different layers of a network. We demonstrate that SelfCon learning improves the classification performance of the encoder network, and empirically analyze its advantages in terms of the single-view and the sub-network. Furthermore, we provide theoretical evidence of the performance increase based on the mutual information bound. For ImageNet classification on ResNet-50, SelfCon improves accuracy by +0.6% with 59% memory and 48% time of Supervised Contrastive learning, and a simple ensemble of multi-exit outputs boosts performance up to +1.5%. Our code is available at https://github.com/raymin0223/self-contrastive-learning.

==> Tables/ablation_resnet50.tex <==
\begin{table}[!t]
\caption{\textbf{The results of SelfCon-S loss according to the structure and position of sub-network.} The classification accuracy is for ResNet-50 on the CIFAR-100 benchmark.}
\scriptsize
\centering
\label{tab:ablation_resnet50}
% \setlength{\tabcolsep}{10pt}
% \renewcommand{\arraystretch}{1.3}
\begin{tabular}{lcccc}
\toprule
    & \multicolumn{3}{c}{Position} & \\ \cmidrule(l{2pt}r{2pt}){2-4}
 \multirow{-2.5}{*}{Structure} & $1^{\text{st}}$ Block    &  $2^{\text{nd}}$ Block    &   $3^{\text{rd}}$ Block  & \multirow{-2.5}{*}{Accuracy} \\ \midrule \hline
     FC   &   &   \cmark    &   &  $\mathbf{78.5_{\pm{0.3}}}$ \\
     Small   &   &  \cmark      &   &  $\mathbf{78.1_{\pm{0.2}}}$ \\
     Same   &   &  \cmark      &   &  $77.4_{\pm{0.2}}$ \\ \hline
     FC   & \cmark     &    &   &  $77.0_{\pm{0.2}}$ \\
     FC   &   &  \cmark  &   &  $\mathbf{78.5_{\pm{0.3}}}$ \\
     FC   &   &   & \cmark    &  $77.4_{\pm{0.1}}$ \\
     FC   & \cmark  &  \cmark  & \cmark  &  $\mathbf{78.7_{\pm{0.5}}}$ \\ \bottomrule
\end{tabular}
\end{table}

==> Tables/ablation_vgg.tex <==
\begin{table}[!t]
\caption{\textbf{The results of SelfCon-S loss according to the structure and position of sub-network.} The classification accuracy is for VGG-16 with BN on the CIFAR-100 benchmark.}
\scriptsize
\centering
\label{tab:ablation_vgg}
% \setlength{\tabcolsep}{10pt}
% \renewcommand{\arraystretch}{1.3}
\begin{tabular}{lccccc}
\toprule
    & \multicolumn{4}{c}{Position} & \\ \cmidrule(l{2pt}r{2pt}){2-5}
 \multirow{-2.5}{*}{Structure} & $1^{\text{st}}$ Block    &  $2^{\text{nd}}$ Block    &   $3^{\text{rd}}$ Block & $4^{\text{th}}$ Block  & \multirow{-2.5}{*}{Accuracy} \\ \midrule \hline
     FC   &   &   \cmark &    &   &  $\mathbf{71.4_{\pm{0.0}}}$ \\
     Small   &   &  \cmark  &    &   &  $\mathbf{71.5_{\pm{0.4}}}$ \\
     Same   &   &  \cmark   &   &   &  $\mathbf{71.5_{\pm{0.3}}}$ \\ \hline
     FC   & \cmark &    &  &   &  $70.9_{\pm{0.1}}$ \\
     FC   &   &  \cmark  &   & & $71.4_{\pm{0.0}}$ \\
     FC   &   &   & \cmark &   &  $72.0_{\pm{0.0}}$ \\
     FC   &   &   &  & \cmark  &  $71.5_{\pm{0.1}}$ \\
     FC   & \cmark  &  \cmark  & \cmark  & \cmark & $\mathbf{72.5_{\pm{0.1}}}$ \\ \bottomrule
\end{tabular}
\end{table}

==> Tables/ensemble.tex <==
\begin{table}[!t]
    \centering
    \scriptsize 
    \caption{\textbf{Classification accuracy with the classifiers after backbone, sub-network, and the ensemble of them.} The ResNet-18 encoder is pretrained by the SelfCon-S loss function. CF and IN indicate CIFAR and ImageNet, respectively. Refer to Appendix \ref{app:ensemble_resnet50} for the results on ResNet-50.}
    \label{tab:subnet_ensemble}
    \resizebox{\linewidth}{!}{
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{lccccc}
    \toprule
    Method & CF-10 & CF-100 & Tiny-IN & IN-100 & IN  \\ \midrule \hline
    SupCon & $94.7$ & $73.0$ & $56.9$ & $85.5$ & $71.2$ \\ \hline
    Backbone & $\mathbf{95.3}$  & $75.4$ &  $59.8$ & $86.3$ & $71.5$ \\
    Sub-network & $92.6$  & $69.1$ & $53.5$ & $85.0$ & $71.2$  \\
    Ensemble & $95.2$ & $\mathbf{77.4}$ &  $\mathbf{62.2}$ & $\mathbf{87.2}$ & $\mathbf{72.6}$  \\
    \bottomrule
    \end{tabular}}
    \vspace{-0.2in}
\end{table}

==> Tables/imagenet.tex <==
\begin{table}
\centering
\small
 \caption{\textbf{The classification accuracy on ResNet-18 for ImageNet.} The performance of CE is reported only in $B=1024$. Every memory and time is reported by comparing to those of SelfCon-S in each batch size.}
 \label{tab:imagenet}
 \vspace{-0.1in}
\centering
\resizebox{\linewidth}{!}{
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{$B=1024$} & \multicolumn{3}{c}{$B=2048$} \\ 
\cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7}
\multirow{-2.5}{*}{Method} & Mem. & Time & Acc@1 & Mem. & Time & Acc@1 \\ \midrule \hline
CE & - & - & $69.4$ & - & - & $69.4$ \\  
\hline
SupCon & $\times 1.6$ & $\times 2.2$ & $70.9$ & $\times 1.5$ & $\times 2.2$ & $71.2$ \\
SupCon-S & $\times \mathbf{0.9}$ & $\times \mathbf{1.0}$ & $69.2$ & $\times \mathbf{0.9}$ & $\times \mathbf{1.0}$ & $70.2$ \\
\rowcolor[gray]{.8}
SelfCon-M & $\times 1.7$ & $\times 2.3$ & $\mathbf{71.2}$ & $\times 1.7$ & $\times 2.3$ & $\mathbf{71.6}$ \\
\rowcolor[gray]{.8}
SelfCon-S & \underline{$\times 1.0$} & \underline{$\times \mathbf{1.0}$} & $70.3$ & \underline{$\times 1.0$} & \underline{$\times \mathbf{1.0}$} & $71.5$ \\
\bottomrule
\end{tabular}}
\vspace{-0.2in}
\end{table}

==> Tables/imagenet100.tex <==
\begin{table}
\centering
\small
 \caption{\textbf{The classification accuracy on ResNet-18 and ResNet-50 for ImageNet-100.} %Parentheses indicate the performance of ensemble prediction in the multi-exit framework (refer to Section \ref{exp:subnetwork}). 
 We summarized the ratio of memory (GiB / GPU) and Time (sec / step) based on those of SelfCon-S in each backbone.}
 \label{tab:imagenet100}
 \vspace{-0.1in}
\resizebox{\linewidth}{!}{
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{ResNet-18} & \multicolumn{3}{c}{ResNet-50} \\ \cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7}
\multirow{-2.5}{*}{Method} & Mem. & Time & Acc@1 & Mem. & Time & Acc@1 \\ \midrule \hline
CE & - & - & $83.7$ & - & - & $86.4$ \\  
\hline
SupCon & $\times 1.5$ & $\times 2.1$ & $85.5$ & $\times 1.7$ & $\times 1.7$ & $88.2$ \\
SupCon-S & $\times \mathbf{1.0}$ & $\times \mathbf{1.0}$ & $84.9$ & $\times \mathbf{0.9}$ & $\times \mathbf{0.8}$ & $87.8$ \\
\rowcolor[gray]{.8}
SelfCon-M & $\times 1.6$ & $\times 2.1$ & $85.8$ & $\times 1.8$ & $\times 2.2$ & $\mathbf{88.9}$ \\
\rowcolor[gray]{.8}
SelfCon-S & \underline{$\times \mathbf{1.0}$} & \underline{$\times \mathbf{1.0}$} & $\mathbf{86.3}$ & \underline{$\times 1.0$} & \underline{$\times 1.0$} & $88.5$ \\
\bottomrule
\end{tabular}}
\vspace{-0.1in}
\end{table}

==> Tables/imagenet_large.tex <==
\begin{minipage}{\textwidth}
\begin{minipage}[!t]{0.48\textwidth}
\centering
\small
% \vspace*{-0.1in}
\captionof{table}{\textbf{The classification accuracy for ImageNet-100.} %Parentheses indicate the performance of ensemble prediction in the multi-exit framework (refer to Section \ref{exp:subnetwork}). 
The performance is reported in $B=512$.
We summarized the ratio of memory (GiB / GPU) and time (sec / step) based on those of SelfCon-S in each backbone.} \label{tab:imagenet100}
% \vspace{-0.1in}
\resizebox{\linewidth}{!}{
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{ResNet-18} & \multicolumn{3}{c}{ResNet-50} \\ \cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7}
\multirow{-2.5}{*}{Method} & Mem. & Time & Acc@1 & Mem. & Time & Acc@1 \\ \midrule \hline
CE & - & - & $83.7$ & - & - & $86.4$ \\  
\hline
SupCon & $\times 1.5$ & $\times 2.1$ & $85.5$ & $\times 1.7$ & $\times 1.7$ & $88.2$ \\
SupCon-S & $\times \mathbf{1.0}$ & $\times \mathbf{1.0}$ & $84.9$ & $\times \mathbf{0.9}$ & $\times \mathbf{0.8}$ & $87.8$ \\
\rowcolor[gray]{.8}
SelfCon-M & $\times 1.6$ & $\times 2.1$ & $85.8$ & $\times 1.8$ & $\times 2.2$ & $\mathbf{88.7}$ \\
\rowcolor[gray]{.8}
SelfCon-S & \underline{$\times \mathbf{1.0}$} & \underline{$\times \mathbf{1.0}$} & $\mathbf{86.3}$ & \underline{$\times 1.0$} & \underline{$\times 1.0$} & $88.5$ \\
\bottomrule
\end{tabular}}
\end{minipage}
\hfill
\begin{minipage}[!t]{0.48\textwidth}
\centering
\small
% \vspace*{-0.1in}
\captionof{table}{\textbf{The classification accuracy for ImageNet.} The performance is reported in $B=2048$. Every memory and time is reported by comparing to those of SelfCon-S. Refer to Appendix \ref{app:ablation_studies} for ResNet-50 results.} \label{tab:imagenet}
%  \vspace{-0.1in}
\centering
\resizebox{\linewidth}{!}{
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{ResNet-18} & \multicolumn{3}{c}{ResNet-34} \\ 
\cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7}
\multirow{-2.5}{*}{Method} & Mem. & Time & Acc@1 & Mem. & Time & Acc@1 \\ \midrule \hline
CE & - & - & $69.4$ & - & - & $72.7$ \\  
\hline
SupCon & $\times 1.5$ & $\times 2.2$ & $71.2$ & $\times 1.5$ & $\times 2.1$ & $74.9$ \\
SupCon-S & $\times \mathbf{0.9}$ & $\times \mathbf{1.0}$ & $70.2$ & $\times \mathbf{0.9}$ & $\times \mathbf{1.0}$ & $74.4$ \\
\rowcolor[gray]{.8}
SelfCon-M & $\times 1.7$ & $\times 2.3$ & $\mathbf{71.6}$ & $\times 1.7$ & $\times 2.2$ & $75.5$ \\
\rowcolor[gray]{.8}
SelfCon-S & \underline{$\times 1.0$} & \underline{$\times \mathbf{1.0}$} & $71.5$ & \underline{$\times 1.0$} & \underline{$\times \mathbf{1.0}$} & $\mathbf{75.6}$ \\
\bottomrule
\end{tabular}}
\end{minipage}
\end{minipage}

% \begin{minipage}{\textwidth}
% \begin{minipage}[!t]{0.45\textwidth}
% \centering
% \scriptsize
% \vskip -0.4in
%     \captionof{table}{\textbf{The classification accuracy on ResNet-18 \textcolor{red}{and ResNet-50} for ImageNet-100.} Parentheses indicate the performance of ensemble prediction in the multi-exit framework (refer to Section \ref{exp:subnetwork}). We reported the results with one random seed. \textcolor{red}{Note that Acc@5 shows the same trend of Acc@1.}}
%     \label{tab:imagenet100}
%     \begin{tabular}{lcc}
%     \toprule
%     Method & \textcolor{red}{ResNet-18} & \textcolor{red}{ResNet-50} \\ \hline \hline
%     CE & $81.1$  & \textcolor{red}{$82.3$} \\  
%     \hline
%     SupCon & $83.0$  & \textcolor{red}{$86.3$} \\
%     SupCon-S & $83.5$  & \textcolor{red}{$86.8$}  \\
%     SelfCon-M & $83.9_{(85.9)}$ &  \textcolor{red}{$86.8_{(88.1)}$}  \\
%     SelfCon-S & $\mathbf{84.5_{(86.0)}}$ & \textcolor{red}{$\mathbf{87.8_{(88.2)}}$} \\ \bottomrule
%     \end{tabular}
% \end{minipage}
% \hfill
% \begin{minipage}[!t]{0.5\textwidth}
% \centering
% \includegraphics[width=.65\textwidth]{Figures/mutual_information/MI_graph.pdf}
% \captionof{figure}{\textbf{Test accuracy and the estimated mutual information of different methods.} Mutual information estimators are measured between the intermediate and the last features.
% }
% \vspace{0.1in}
% \label{fig:mi_connect}
% \end{minipage}
% \end{minipage}

==> Tables/imagenet_various_batch.tex <==
% \begin{wraptable}{R}{6cm}
% \vspace{-0.2in}
% \centering
% \small
%     \caption{\textbf{The classification accuracy for ImgaeNet with 3072 batch size.} We used a ResNet-18 architecture. \xmark\,denotes the failure of the convergence.}
%     \begin{tabular}{lccc}
%     \toprule
%     Method & Mem. & Time. & Acc@1 \\ \midrule \hline
%     CE  & - & - & $69.4$  \\
%     \hline
%     SupCon & $\times 1.6$ & $\times 2.4$ & $71.2$ \\
%     SupCon-S & $\times \mathbf{0.9}$ & $\times \mathbf{1.0}$ & \xmark \\
%     SelfCon-M & $\times 1.8$ & $\times 2.5$ & $\mathbf{71.7}$ \\
%     SelfCon-S & \underline{$\times 1.0$} & \underline{$\times \mathbf{1.0}$} & $71.3$ \\ \bottomrule
%     \end{tabular}
%     \label{tab:imagenet_large_batch}
% \end{wraptable}

\begin{wraptable}{R}{5.8cm}
\vspace*{-0.2in}
\centering
\small
    \caption{\textbf{The classification accuracy for ImgaeNet with 1024 batch size.} We used a ResNet-18 architecture.}\label{tab:imagenet_small_batch}
    \begin{tabular}{lccc}
    \toprule
    Method & Mem. & Time. & Acc@1 \\ \midrule \hline
    CE  & - & - & $69.4$  \\
    \hline
    SupCon & $\times 1.6$ & $\times 2.1$ & $70.9$ \\
    SupCon-S & $\times \mathbf{1.0}$ & $\times \mathbf{1.0}$ & $69.2$ \\
    SelfCon-M & $\times 1.5$ & $\times 2.1$ & $\mathbf{71.2}$ \\
    SelfCon-S & \underline{$\times 1.0$} & \underline{$\times \mathbf{1.0}$} & $70.3$ \\ \bottomrule
    \end{tabular}
\vspace*{-10pt}
\end{wraptable}

==> Tables/learning_rate_imagenet.tex <==
\begin{wraptable}{r}{6.5cm}
\centering
\small
\vspace*{-20pt}
\caption{\textbf{ImageNet results on ResNet-18 with various learning rates.} \textbf{Bold} type is for the best accuracy within each method. We used a \textit{same} sub-network structure for SelfCon.}
\vspace{-3pt}
\label{tab:learning_rate_imagenet}
    \begin{tabular}{lcccc}
    \toprule
    & \multicolumn{4}{c}{Learning Rate} \\
    \cmidrule(l{2pt}r{2pt}){2-5}
    \multirow{-2.5}{*}{Method} & $0.1875$ & $0.375$ & $0.75$ & $1.5$ \\
    \midrule\hline
    SupCon & $71.0$ & $\mathbf{71.2}$ & $\mathbf{71.2}$ & $70.7$ \\
    SelfCon &  $\mathbf{71.3}$ & $\mathbf{71.3}$ & $71.1$ & $69.1$ \\ \bottomrule
    \end{tabular}
\vspace*{-20pt}
\end{wraptable}

==> Tables/lr_cf100_in100.tex <==
\begin{table}[!t]
\begin{minipage}[!t]{0.48\textwidth}
\end{minipage}
\end{table}

\begin{wraptable}{r}{8.5cm}
\centering
\small
\vspace{-0.15in}
\caption{\textbf{CIFAR-100 results on ResNet-18 with various learning rates.} \textbf{Bold} type is for the best accuracy within each method. We used a fully-connected layer (to be defined as \textit{fc}) as the sub-network for SelfCon methods.}
\label{tab:sensitivity_study}
    \begin{tabular}{lcccccc}
    \toprule
    & \multicolumn{6}{c}{Learning Rate} \\
    \cmidrule(l{2pt}r{2pt}){2-7}
    \multirow{-2.5}{*}{Method} & $0.125$ & $0.25$ & $0.5$ & $1.0$ & $2.0$ & $4.0$ \\
    \midrule\hline
    SupCon & $71.8$ & $72.3$ & $73.0$ & $73.4$ & $74.6$ & $\mathbf{74.7}$ \\
    SupCon-S & $72.3$ & $73.1$ & $73.9$ & $74.6$ & $\mathbf{74.8}$ & $73.6$ \\
    SelfCon-M & $72.3$ & $73.6$ & $74.9$ & $\mathbf{75.5}$ & $\mathbf{75.5}$ & $75.1$ \\
    SelfCon-S &  $74.3$ & $74.6$ & $75.4$ & $75.7$ & $\mathbf{76.0}$ & $74.7$ \\ \bottomrule
    \end{tabular}
    \vspace{-0.1in}
\end{wraptable}


\begin{wraptable}{r}{8.5cm}
\centering
\vspace{-0.15in}
\small
\caption{\textbf{ImageNet-100 results on ResNet-18 with various learning rates.} \textbf{Bold} type is for the best accuracy within each method. For sub-network structure on the SelfCon methods, non-sharing blocks of the backbone and sub-network are the same (to be defined as \textit{same}).}
\label{tab:learning_rate_imagenet100}
    \begin{tabular}{lcccccc}
    \toprule
    & \multicolumn{6}{c}{Learning Rate} \\
    \cmidrule(l{2pt}r{2pt}){2-7}
    \multirow{-2.5}{*}{Method} & $0.125$ & $0.25$ & $0.5$ & $1.0$ & $2.0$ & $4.0$ \\
    \midrule\hline
    SupCon & $83.4$ & $84.5$ & $85.2$ & $\mathbf{85.5}$ & $84.3$ & $75.4$ \\
    SupCon-S & $83.8$ & $84.7$ & $\mathbf{84.9}$ & $84.8$ & $82.3$ & $1.0$ \\
    SelfCon-M & $84.6$ & $85.2$ & $\mathbf{85.8}$ & $85.5$ & $84.8$ & $73.4$ \\
    SelfCon-S &  $84.8$ & $85.4$ & $\mathbf{85.7}$ & $85.4$ & $84.0$ & $56.3$ \\ \bottomrule
    \end{tabular}
    \vspace{-0.1in}
\end{wraptable}

==> Tables/mutual_information.tex <==
\begin{table}[!t]
\small
\centering
\caption{\textbf{The detailed results of mutual information estimation in Figure \ref{fig:mi_connect}.} $\vx$, $\vy$, $\mT(\vx)$, and $\mF(\vx)$ respectively denotes the input variable, label variable, intermediate feature, and the last feature. Recall that $\mT(\vx)$ is the intermediate feature of the backbone network, which is an input to the auxiliary network path. We summarized the average of estimated MI through multiple random seeds. We highlighted the MI between the intermediate and the last features, which is the main concern of the SelfCon loss. \textbf{Bold} type indicates the smallest values for $\gI(\vx;\mT(\vx))$ and the largest values for $\gI(\vy;\mT(\vx))$ and $\gI(\mF(\vx);\mT(\vx))$, according to the IB principle.}
\label{tab:detail_mi}
\begin{tabular}{llcccc}
\toprule
Estimator & MI & CE & SupCon & SelfCon-M & SelfCon-S \\ 
\midrule\hline
%
& $\gI(\vx;\mT(\vx))$ & $0.509$ & $0.344$ & $\mathbf{0.231}$ & $0.236$  \\ 
& $\gI(\vy;\mT(\vx))$ & $0.214$ & $0.235$ & $0.469$ & $\mathbf{0.479}$ \\
\rowcolor[gray]{.8}
\cellcolor{white}  \multirow{-3}{*}{InfoNCE \citep{cpc}} & $\gI(\mF(\vx);\mT(\vx))$ & $0.288$ & $0.303$ & $0.530$ & $\mathbf{0.553}$ \\ \hline
%
& $\gI(\vx;\mT(\vx))$ & $1.639$ & $0.898$ & $0.558$ & $\mathbf{0.554}$ \\
& $\gI(\vy;\mT(\vx))$ & $0.398$ & $0.627$ & $1.486$ & $\mathbf{1.680}$ \\
\rowcolor[gray]{.8}
\cellcolor{white} \multirow{-3}{*}{MINE \citep{mine}} & $\gI(\mF(\vx);\mT(\vx))$ & $0.734$ & $0.762$ & $1.726$ & $\mathbf{2.123}$ \\ 
\hline
%
& $\gI(\vx;\mT(\vx))$ & $1.485$ & $0.930$ & $0.601$ & $\mathbf{0.589}$ \\ 
& $\gI(\vy;\mT(\vx))$ & $0.390$ & $0.546$ & $\mathbf{1.450}$ & $1.389$ \\
\rowcolor[gray]{.8}
\cellcolor{white}  \multirow{-3}{*}{NWJ \citep{nwj}} & $\gI(\mF(\vx);\mT(\vx))$ & $0.655$ & $0.799$ & $1.820$ & $\mathbf{1.873}$ \\
 \bottomrule
\end{tabular}
\end{table}
